Quantum Control at the Boundary

This dissertation presents and prove the viability of a non-standard method for controlling the state of a quantum system by modifying its boundary conditions instead of relying on the action of external fields. The standard approach to quantum control bases on the use of an external field to manipulate the system. Some technological difficulties appear when controlling a quantum system in this way, due to the complications of manipulating a system made of few particles while maintaining the quantum correlations. As a consequence the systems need to be kept at very low temperatures and the interactions have to be performed very fast. The Quantum Control at the Boundary approach is radically different to the standard one. Instead of seeking the control of the quantum system by directly interacting with it through an external field, the control is achieved by manipulating the boundary conditions of the system. The spectrum of a quantum system, for instance an electron moving in a box, depends on the boundary conditions imposed on it. Hence, a modification of such boundary conditions modifies the state of the system allowing for its manipulation and, eventually, its control. This kind of interaction is weaker, which makes one to expect that it may help maintaining the quantum correlations. For showing the viability of the Quantum Control at the Boundary method, a family of boundary control systems on Quantum Circuits (a generalization of quantum grahs) is introduced. Before being able to address the problem of controllability, the problem of existence of solutions for the Schr\"odinger equation with time-dependent boundary conditions is addressed. The approximate controllability of the systems under study is proven using a controllability result by T. Chambrion et al. (2009) and a stability result which constitutes another original contribution of this dissertation.

==> portada.tex <==
%auto-ignore
\thispagestyle{empty}
\begin{center}

~
\mbox{\parbox{3cm} {\centering\scriptsize\mbox{\includegraphics[width=3.2cm]{img/logouc3m.pdf}}}}
%\mbox{\parbox{2cm} {\centering\scriptsize\mbox{\includegraphics[width=2cm] {logouc3m-azul}}}}

\vspace{0.5cm}

{\large UNIVERSIDAD CARLOS III DE MADRID}

\vspace{0.75cm}



{\Large TESIS DOCTORAL} \vspace{0.75cm}



\rule{\linewidth}{0.2mm}

\vspace*{2.8mm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

{\Large\textsc{\textbf{ \thetitle }}}
\rule{\linewidth}{0.2mm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\vspace{1cm}


{\textbf{Autor: }}

\vspace{1mm}

{\textbf{\theauthor}}

\vspace{3mm}

%{\large\textbf{DIRECTOR: ALBERTO IBORT LATRE}} \vspace{2cm}
{\textbf{Directores:}}

\vspace{1mm}

{\textbf{\theadvisors}}

\vspace{1.5cm}

{\large  DEPARTAMENTO DE MATEM\'ATICAS} \vspace{5mm}

{\large \textrm{Legan\'es, 2021}}
\end{center}

%\clearemptydoublepage

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newpage\thispagestyle{empty}

{\center
{\large Firma del Tribunal Calificador} \vspace{1cm}

%\begin{table}
\begin{tabular}[h]{l | c | r}
	  &\phantom{aaaaaaaaaaaaaaaaaaaaaaaaaaaaaaaaaaaaaaaaaaa} &{\large Firma}\phantom{aaaaaaaa}\\ \hline
	& &\\
	{\large Presidente:}& & \\
	 & &\\ \hline
	  & &\\
	{\large Vocal:} & &\\
	 & & \\ \hline
	 & &\\
	{\large Secretario: } & &\\
	& &\\ \hline
\end{tabular}
%\end{table}

\vspace{2cm}

{\large Calificaci\'{o}n\;:}
}
\vspace{2cm}

\begin{center}
{Legan\'{e}s, \phantom{aaaaaaa}de \phantom{aaaaaaaaaaaaaaaaaaaaaaaaaaaaaaaaa} de}
\end{center}

